Second-Order Hyperproperties

We introduce Hyper$^2$LTL, a temporal logic for the specification of hyperproperties that allows for second-order quantification over sets of traces. Unlike first-order temporal logics for hyperproperties, such as HyperLTL, Hyper$^2$LTL can express complex epistemic properties like common knowledge, Mazurkiewicz trace theory, and asynchronous hyperproperties. The model checking problem of Hyper$^2$LTL is, in general, undecidable. For the expressive fragment where second-order quantification is restricted to smallest and largest sets, we present an approximate model-checking algorithm that computes increasingly precise under- and overapproximations of the quantified sets, based on fixpoint iteration and automata learning. We report on encouraging experimental results with our model-checking algorithm, which we implemented in the tool~\texttt{HySO}.

==> InputFigures/common-knowledge-architecture.tex <==
\tikzstyle{state}=[draw, rectangle, fill=none, minimum width=.8cm, 
minimum height = .8cm, rounded corners=1mm, align=center, thick]

\begin{tikzpicture}[->,>=stealth',shorten >= 1pt,auto]

\node[state, fill=gray!30] (p1) {%
  $~p_1$
};
%\node (left) [left =0.7 of p1]{};

\node[state,fill=gray!30] (p2) [right= 1.1 of p1] {%
  $~p_2$};
%\node[state, draw= none] (p3) [right= 1 of p2] {%
%  $...$};
%\node[state] (p4) [right= 1 of p3] {%
%  $p_n$};
%\node (right) [right = 0.7 of p4] {};
\node[state] (env1) [draw=none, above = .7 of p1]{};
\node[state] (env2) [draw=none, above = .7 of p2]{};

\node[state, draw = none, minimum height=.1cm] (p1below) [below= .7 of p1] {%
 % $p_2$
 };
\node[state, draw = none, minimum height=.1cm] (p2below) [below= .7 of p2] {%
%  $p_2$
 };
%\node[state, draw = none, minimum height=.1cm] (p3below) [below= .5 of p3] {%
%  $...$
%};
%\node[state, draw = none, minimum height=.1cm] (p4below) [below= .5 of p4] {%
%  $p_n$
%};

\node (phantom) [below =1.2 of p1, draw = none]{\phantom{test}};
\path (env1) edge[thick, transform canvas={yshift=0mm}] node[above left, yshift=-1mm] {%
        $i_{p_1}$
      } node[above right, yshift=-1mm] {%
        $e_{p_1}$
      }
      (p1)
      (env2) edge[thick, transform canvas={yshift=0mm}] node[above right, yshift=-1mm] {%
        $i_{p_2}$
      }  
      node[above left, yshift=-1mm] {%
        $e_{p_2}$
      }(p2)
      %(env) edge[thick, transform canvas={yshift=0mm}] node[left] {%
      %  $...$
      %}  (p3)
      %(env) edge[thick, transform canvas={yshift=0mm}] node[right] {%
      %  $\vin_{p_n}$
      %}  (p4)
      %(p1) edge[transform canvas={yshift=-1.5mm}] node[below] {%
      %  $\vouta$
      %}  (left)
      (p1) edge[thick, transform canvas={yshift=1.5mm}] node[above] {%
        $c_{p_1}$
      } (p2)
      (p2) edge[thick, transform canvas={yshift=-1.5mm}] node[below] {%
        $c_{p_2}$
      } (p1)
      %(p2) edge[thick, transform canvas={yshift=0mm}] node[above] {%
      %  $\vc$
      %} (p3)
      %(p3) edge[thick, transform canvas={yshift=0mm}] node[above] {%
      %  $\vc$
      %} (p4)
      %(p2) edge[transform canvas={yshift=-1.5mm}] node[below] {%
      %  $\vcba$
      %} (p1)
      %(p4) edge[thick, transform canvas={yshift=0mm}] %node[above] {
      %$\vout$
      %}(right)
      (p1) edge[thick, transform canvas={yshift=0mm}] node[left] {
      $o_{p_1}$
      }(p1below)
      (p2) edge[thick, transform canvas={yshift=0mm}] node[right] {
      $o_{p_2}$
      }(p2below)
      %(p3) edge[thick, transform canvas={yshift=0mm}] node[right] {
      %$...$
      %}(p3below)
      %(p4) edge[thick, transform canvas={yshift=0mm}] node[right] {
      %$\vout_{p_4}$
      %}(p4below)
      %(right) edge[transform canvas={yshift=1.5mm}] node[above] {
      %$\vinb$
      %}(p2)
      ;
\end{tikzpicture}

==> InputFigures/common-knowledge-p2.tex <==
\tikzstyle{state}=[draw, circle, fill=none, minimum width=1cm, 
minimum height = 1cm, align=center, thick]

\begin{tikzpicture}[->,>=stealth',shorten >= 1pt,auto]

\node[state] (s0) [scale=1.2]{%
    $p_2$\\
    $s_0$
};

\node (left) [left = 0.5 of p1, draw=none]{};

\node[state] (s1) [right =  3 of p1] {%
    $p_2$\\
  $s_1$
 };

 \node[state] (s2) [below right = 1.2 and 1.5 of p1] {%
    $p_2$\\
  $s_2$
 };


 %\node (right) [right = 0.5 of p2, draw=none]{};

%\node[state] (p2) [below right= .1 and 1.5 of p0]{
%    $b_2$\\
%    $\neg o$
%    };

%\node[state] (p3) [right = 3 of p0, draw=none] {%
%    $\phantom{b_3}$\\
%    $\phantom{o}$
%  };
  

\path (left) edge (s0)
      (s0) edge[thick, bend left=20, align=center] node[above, sloped] {%
        $i_{p_2} \wedge  e_{p_2} /$
      $c_{p_2}$
      } (s1)
      (s0) edge[thick, bend left=18, align=center] node[above,sloped] {%
        $\neg i_{p_2} / \neg c_{p_2}$
      } (s2)
      (s0) edge[thick, bend right=18, align=center] node[sloped,below] {%
        $i_{p_2} \wedge \neg e_{p_2} /$
        $ c_{p_2} $
      } (s2)
      (s1) edge[thick, bend left=18, align=center] node [sloped, below] {%
     $c_{p_1} / \neg o_{p_2}$
      }(s2)
      (s1) edge[thick, bend right=18, align=center] node [above , sloped] {%
     $\neg c_{p_1} /$
     $ \neg o_{p_2}$
      }(s2)
      (s2) edge[loop below, thick, align=center] node [below] {%
      $* / \neg o_2$
      }(s2)
      %(p3) edge[loop right, thick, draw=none] node [right] {%
      %$\phantom{\LTLtrue}$}(p3)
      ;
\end{tikzpicture}
